MRAC with Memory for Switched Linear Systems

This work proposes a switched model reference adaptive control (S-MRAC) architecture for a multi-input multi-output (MIMO) switched linear system with memory for enhanced learning. A salient feature of the proposed method that separates it from most previous results is the use of memory that store the estimator states at switching and facilitate parameter learning during both active and inactive phases of a subsystem, thereby improving the tracking performance of the overall switched system. Specifically, the learning experience from the previous active duration of a subsystem is retained in the memory and reused when the subsystem is inactive and when the subsystem becomes active again. Parameter convergence is shown based on an intermittent initial excitation (IIE), which is significantly relaxed than the classical persistence of excitation (PE) condition. A common Lyapunov function is considered to ensure closed-loop stability with S-MRAC. Further under IIE, the exponential stability of tracking and parameter estimation error dynamics are guaranteed.

==> bibliography.tex <==


\begin{thebibliography}{}
\bibitem{c1} Wang, Wei and Wen, Changyun, "Adaptive compensation for infinite number of actuator failures or faults", \textit{Automatica}, vol. 47, no. 10, pp.2197--2210, 2011

\bibitem{c2} Zhang, Jin-Xi and Yang, Guang-Hong, "Fault-tolerant output-constrained control of unknown Euler--Lagrange systems with prescribed tracking accuracy", \textit{Automatica}, vol.111, pp. 108606, 2020

\bibitem {c3} Tao, Gang and Joshi, Suresh M and Ma, Xiaoli, "Adaptive state feedback and tracking control of systems with actuator failures" \textit{IEEE Transactions on Automatic Control}, vol.46, no. 1 pp.78--95, 2001

\bibitem {c4} Dawson, Darren M and Carroll, James J and Schneider, M, "Integrator backstepping control of a brush DC motor turning a robotic load" \textit{IEEE Transactions on Control Systems Technology}, vol.2, no. 3 pp.233--244, 1994

\bibitem {c5} Dupree, Keith and Patre, Parag M and Wilcox, Zachary D and Dixon, Warren E "Integrator backstepping control of a brush DC motor turning a robotic load" \textit{Automatica}, vol.47, no. 1 pp.99--107, 2011

\bibitem {c6} Patre, PM and MacKunis, W and Kaiser, K and Dixon, WE "Asymptotic tracking for uncertain dynamic systems via a multilayer NN feedforward and RISE feedback control structure" \textit{2007 American Control Conference}, pp.5989--5994, 2007

\bibitem{c7}Sharma, Nitin and Bhasin, Shubhendu and Wang, Qiang and Dixon, Warren E, "Predictor-based control for an uncertain Euler--Lagrange system with input delay", \textit{Automatica}, vol.47, no.11, pp.2332--2342, 2011

\bibitem{c8}Song, Yongduan and Guo, Junxia "Neuro-adaptive fault-tolerant tracking control of Lagrange systems pursuing targets with unknown trajectory", \textit{IEEE Transactions on Industrial Electronics}, vol.64, no.5, pp.3913--3920, 2016

\bibitem{c9}Tang, Xidong and Tao, Gang and Joshi, Suresh M, "Adaptive actuator failure compensation for parametric strict feedback systems and an aircraft application" \textit{Automatica}, vol.39, no.11, pp.1975--1982, 2003

\bibitem{c10}Yang, Qinmin and Ge, Shuzhi Sam and Sun, Youxian, "Adaptive actuator fault tolerant control for uncertain nonlinear systems with multiple actuators" \textit{Automatica}, vol.60, no.11, pp.92--99, 2015

\bibitem{c11} Jin, Xu "Fault tolerant nonrepetitive trajectory tracking for MIMO output constrained nonlinear systems using iterative learning control" \textit{IEEE transactions on cybernetics}, vol.49, no.8, pp.3180--3190, 2018

\bibitem{c12} Song, Yongduan and Guo, Junxia "Neuro-adaptive fault-tolerant tracking control of Lagrange systems pursuing targets with unknown trajectory" \textit{IEEE Transactions on Industrial Electronics}, vol.64, no.5, pp.3913--3920, 2016

\bibitem{c13} Zhang, Jin-Xi and Yang, Guang-Hong, "Fault-tolerant leader-follower formation control of marine surface vessels with unknown dynamics and actuator faults", \textit{International Journal of Robust and Nonlinear Control}, vol. 28, no. 14, pp. 4188--4208, 2018

\bibitem{c14} Gao, Hui and Song, Yongduan and Wen, Changyun, "Backstepping design of adaptive neural fault-tolerant control for MIMO nonlinear systems", \textit{IEEE transactions on neural networks and learning systems}, vol. 28, no. 11, pp. 2605--2613, 2016

\bibitem{c15} Tao, Gang and Chen, Shuhao and Tang, Xidong and Joshi, Suresh M "Adaptive control of systems with actuator failures", 2013

\bibitem{c16} Wang, Wei and Wen, Changyun "Adaptive actuator failure compensation control of uncertain nonlinear systems with guaranteed transient performance" \textit{Automatica}, vol. 46, no. 12, pp. 2082--2091, 2010

\bibitem{c17} Gao, Zhiwei and Ding, Steven X "Actuator fault robust estimation and fault-tolerant control for a class of nonlinear descriptor systems" \textit{Automatica}, vol. 43, no. 5, pp. 912--920, 2007

\bibitem{c18} Gao, Hui and Song, Yongduan and Wen, Changyun "Backstepping design of adaptive neural fault-tolerant control for MIMO nonlinear systems" \textit{IEEE transactions on neural networks and learning systems}, vol. 28, no. 11, pp. 2605--2613, 2016

\bibitem{c19} Jin, Xu "Fault tolerant finite-time leader--follower formation control for autonomous surface vessels with LOS range and angle constraints" \textit{Automatica}, vol. 68, pp. 228--236, 2016

\bibitem{c20} Lan, Jianglin and Patton, Ron J "A new strategy for integration of fault estimation within fault-tolerant control" \textit{Automatica}, vol. 69, pp. 48--59, 2016

\bibitem{c21} Zhang, Jin-Xi and Yang, Guang-Hong "Prescribed performance fault-tolerant control of uncertain nonlinear systems with unknown control directions" \textit{IEEE Transactions on Automatic Control}, vol. 62, no. 12,  pp. 6529--6535, 2017

\bibitem{c22} Zhang, Jin-Xi and Yang, Guang-Hong "Robust adaptive fault-tolerant control for a class of unknown nonlinear systems" \textit{IEEE Transactions on Industrial Electronics}, vol. 64, no. 1,  pp. 585--594, 2016

\bibitem{c23} Boskovic, Jovan D and Mehra, Raman K, "A decentralized scheme for accommodation of multiple simultaneous actuator failures", \textit{Proceedings of the 2002 American Control Conference (IEEE Cat. No. CH37301)}, vol. 6, pp. 5098--5103, 2002

\bibitem{c24} Tao, Gang and Chen, Shuhao and Joshi, Suresh M, "An adaptive actuator failure compensation controller using output feedback", \textit{IEEE Transactions on Automatic Control}, vol.47, no.3, pp.506--511, 2002

\bibitem{c25} Niemann, Henrik and Stoustrup, Jakob, "Passive fault tolerant control of a double inverted pendulum—a case study", \textit{Control engineering practice}, vol. 13, no.8, pp.1047--1059, 2005

\bibitem{c26} Veillette, Robert J and Medanic, Jure V and Perkins, William R, "Design of reliable control systems",\textit{29th IEEE Conference on Decision and Control}, pp. 1131--1136, 1990

\bibitem{c27} Zhao, Q and Jiang, J,"Reliable state feedback control system design against actuator failures", \textit{Automatica}, vol.34, no. 10, pp. 1267--1272, 1998

\bibitem{c28} Yang, Guang-Hong and Wang, Jian Liang and Soh, Yeng Chai, "Reliable H∞ controller design for linear systems", \textit{Automatica}, vol.37, no. 5, pp. 717--725, 2001

\bibitem {c29} Gao, Zhiqiang and Antsaklis, Panos J, "Stability of the pseudo-inverse method for reconfigurable control systems", \textit{international Journal of Control}, vol. 53, no. 3, pp.717--729, 1991


\bibitem{c30} Esna Ashari*, A and Khaki Sedigh, A and Yazdanpanah, MJ, "Reconfigurable control system design using eigenstructure assignment: static, dynamic and robust approaches", \textit{International Journal of Control}, vol. 78, no. 13, pp.1005--1016, 2005

\bibitem{c31} Corradini, Maria Letizia and Orlando, Giuseppe, "Actuator failure identification and compensation through sliding modes" \textit{IEEE Transactions on Control Systems Technology}, vol. 15, no.1, pp. 184--190, 2006

\bibitem {c32} Zhang, Xiaodong and Parisini, Thomas and Polycarpou, Marios M, \textit{Adaptive fault-tolerant control of nonlinear uncertain systems: an information-based diagnostic approach}, vol. 49, no. 8, pp. 1259--1274, 2004

\bibitem{c33} Zhang, Yingwei and Qin, S Joe, "Adaptive actuator/component fault compensation for nonlinear systems", \textit{AIChe Journal}, vol. 54, no.9, pp.2404--2412, 2008

\bibitem{c34} Slotine, Jean-Jacques E and Li, Weiping, "On the adaptive control of robot manipulators", \textit{The international journal of robotics research}, vol.6, no.3, pp.49-59, 1987

\bibitem{c35} Narendra, Kumpati S and Annaswamy, Anuradha M, "Stable adaptive systems", \textit{John Wiley Sons, Inc.}, 1996

\bibitem{c36} Zhang, Youmin and Jiang, Jin, "Bibliographical review on reconfigurable fault-tolerant control systems", \textit{Annual reviews in control}, vol.32, no.2, pp.229--252, 2008

\bibitem{c37} Roy, Sayan Basu and Bhasin, Shubhendu and Kar, Indra Narayan, "Parameter convergence via a novel pi-like composite adaptive controller for uncertain euler-lagrange systems", \textit{2016 IEEE 55th Conference on Decision and Control (CDC)}, pp. 1261--1266, 2016

\bibitem{c38} Spong, Mark W and Vidyasagar, Mathukumalli, "Robot dynamics and control", \textit{John Wiley \& Sons}, 2008

\bibitem{c39} Khalil, Hassan K, "Nonlinear systems", \textit{Upper Saddle River}, 2002

\bibitem{c40} Yang, Qinmin and Ge, Shuzhi Sam and Sun, Youxian, "Adaptive actuator fault tolerant control for uncertain nonlinear systems with multiple actuators", \textit{Automatica}, vol.60, pp.92--99, 2015

\bibitem{c41} Ouyang, Hupo and Lin, Yan, "Adaptive fault-tolerant control for actuator failures: a switching strategy", \textit{Automatica}, vol.81, pp.87-95, 2017









\end{thebibliography}
